Non-Western Perspectives on Web Inclusivity: A Study of Accessibility Practices in the Global South

The Global South faces unique challenges in achieving digital inclusion due to a heavy reliance on mobile devices for internet access and the prevalence of slow or unreliable networks. While numerous studies have investigated web accessibility within specific sectors such as education, healthcare, and government services, these efforts have been largely constrained to individual countries or narrow contexts, leaving a critical gap in cross-regional, large-scale analysis. This paper addresses this gap by conducting the first large-scale comparative study of mobile web accessibility across the Global South. In this work, we evaluate 100,000 websites from 10 countries in the Global South to provide a comprehensive understanding of accessibility practices in these regions. Our findings reveal that websites from countries with strict accessibility regulations and enforcement tend to adhere better to Web Content Accessibility Guidelines (WCAG) guidelines. However, accessibility violations impact different disability groups in varying ways. Blind and low-vision individuals in the Global South are disproportionately affected, as only 40% of the evaluated websites meet critical accessibility guidelines. This significant shortfall is largely due to developers frequently neglecting to implement valid alt text for images and ARIA descriptions, which are essential specification mechanisms in the HTML standard for the effective operation of screen readers.

==> discussion.tex <==
%\csnote{It would be great to have a point of comparison/baseline, i.e., the number of accessibility issues in the typical/popular/western web}\mvnote{agreed. Can you maybe here add a plot comparing with developed region, like ``overall''? how would this plot look like?},


%%%%%%%%%%%%%%%%%%%%%
\section{Discussion}
%%%%%%%%%%%%%%%%%%%%%


% Our study shows that accessibility remains a significant challenge across the Global South with a large proportion of websites failing to comply with \wcag~guidelines. This lag in accessibility compliance highlights substantial barriers to digital inclusion in these regions. One of the key findings is the distinct challenges associated with mobile web accessibility. Given that mobile devices are often the primary means of internet access in the Global South, the high prevalence of mobile-specific violations, such as improper viewport settings and inadequate touch target sizing, underscores the critical need for mobile-first design practices. 
% Additionally, the study highlights the uneven impact of accessibility issues on different user groups. While more websites comply with requirements for users with mobility impairments or low vision, the needs of blind users are largely neglected, with critical violations such as missing link names and alt text being highly prevalent. This disparity points to an urgent need for targeted interventions to address the unique challenges faced by blind users. 

% Another notable finding is the strong correlation between national laws and accessibility compliance. Countries with specific legislation and robust enforcement mechanisms, such as India’s \textit{Rights of Persons with Disabilities Act} and Brazil’s \textit{eMAG - e-Government Accessibility Model}, demonstrate significantly higher adherence to accessibility standards compared to those with weaker or no regulations. This underscores the pivotal role of governance and policy in fostering inclusive digital environments. Despite these insights, the study reveals that there is considerable room for improvement across all regions. Addressing the widespread violations, especially those affecting the most vulnerable groups, will require a combination of stronger regulatory frameworks, developer education, and widespread adoption of accessibility-first design practices. These efforts are critical to bridging the accessibility gap and promoting digital equity across the Global South.



